Green Runner: A tool for efficient deep learning component selection

For software that relies on machine-learned functionality, model selection is key to finding the right model for the task with desired performance characteristics. Evaluating a model requires developers to i) select from many models (e.g. the Hugging face model repository), ii) select evaluation metrics and training strategy, and iii) tailor trade-offs based on the problem domain. However, current evaluation approaches are either ad-hoc resulting in sub-optimal model selection or brute force leading to wasted compute. In this work, we present \toolname, a novel tool to automatically select and evaluate models based on the application scenario provided in natural language. We leverage the reasoning capabilities of large language models to propose a training strategy and extract desired trade-offs from a problem description. \toolname~features a resource-efficient experimentation engine that integrates constraints and trade-offs based on the problem into the model selection process. Our preliminary evaluation demonstrates that \toolname{} is both efficient and accurate compared to ad-hoc evaluations and brute force. This work presents an important step toward energy-efficient tools to help reduce the environmental impact caused by the growing demand for software with machine-learned functionality.

==> extra.tex <==
The integration of machine learning models into software engineering, particularly in applications requiring intelligent capabilities like image recognition, object detection, and content generation, has been a transformative development. These capabilities, made accessible through APIs and libraries, have expanded the potential of software applications. However, the inclusion of machine learning models has led to increased resource demands, escalating costs, and elongating development times. It also adds complexity to software maintenance and amplifies the environmental impact.
In software engineering selecting models extends beyond simply choosing the highest performing one. Developers need to perform tradeoffs where the decisions are influenced by the specific application scenario, performance and constraints. For example in drones used for monitoring crop health, the optimal model must be lightweight and efficient due to hardware constraints. A less than optimal choice can lead to excessive computational demand, rapidly depleting battery life and reducing operational efficiency. The problem is further complicated when considering the sensitivity of the models, where a model may perform exceptionally in a controlled test environment but could fail to replicate that performance in real-world scenarios where data quality is variable and unpredictable. 
Consider HuggingFace, a large-scale model repository containing 388,608 models, spanning across 32 different tasks where each model requires different hardware, training and evaluation metrics. For instance \autoref{FIG} only shows the computer vision category where we can see the number of valid permutations between tasks, models, metrics, processes and tradeoffs


% too many models, additional constraints
% metrics, tasks , requirments ,models,problem,data.

% The software engineering landscape has changed with the inclusion of machine learning components, embedding applications with intelligent features such as image captioning, image generation, voice recognition and other intelligent features made accessible through API's and libraries. However, the surge in including ML models as components {CITE} poses a significant challenge due to their environmental impact and resource demands scaling with increased development time, costs and impacting maintenance and software evolution {CITE}.


% A growing concern with the popularity of ML in software engineering is its environmental impact and its resource-intensive nature resulting in increased technical debt \cite{tang2021empirical}.
% The problem is the high-dimensional search, evaluating each choice is wasteful and infeasible. Building software applications also requires developers to consider tradeoffs and constraints as a part of the development process which dictates the components which will be used as a part of the final application. Let's consider a model repository such as Hugging Face \footnote{https://huggingface.co/}. Hugging Face has approximately 120k models split across 6 categories and 32 tasks with each model requiring different hardware, training and evaluation metrics. For example, the computer vision category has 8 sub-tasks, with each task having its own evaluation metrics. However, models exist which can perform more than one task, for instance, the Facebook resnet 50 {CITE} can be used for classification and object detection. Therefore a critical question arises of how can developers select and evaluate the right model in a resource-efficient manner and pick the correct metrics to evaluate.

The cost of operating ML models is estimated to be  80\%--90\% of a model's total cost\footnote{https://www.forbes.com/sites/moorinsights/2019/05/09/google-cloud-doubles-down-on-nvidia-gpus-for-inference/} and inefficient use of computing resources contributes to the increased carbon footprint of machine learning (ML) \cite{strubell2019energy} research contributing to the global climate change crisis \cite{masson2018global}.
Selecting resource-efficient models in resource-efficient ways is paramount to reducing the environmental impact of ML and maintaining software evolution and reducing development costs. 

% training a single model has a carbon footprint equivalent to 5 family cars' lifetime emissions~\cite{strubell2019energy}. 

However, model selection is more than selecting the highest-performing model, tradeoffs need to be made in the selection of ML components, which depends on the application scenario or the use case~\cite{Jabbarpour2021} and the quality and availability of data. For example, a model designed to run on a drone to monitor crop health runs on resource-constrained hardware whereas a suboptimal model will consume higher compute draining the battery faster and reducing flight time. In comparison, a model operating in an autonomous vehicle has no hardware limitations although should have low latency to detect hazards in a timely manner, and a sub-optimal model could be the difference between life and death \cite{inbook}. On the other hand, if a model is sensitive to the data, may boast high performance in a test setting, however, the model will under-perform in a real-world scenario where data quality cannot be determined.
%In the case of autonomous vehicles a 1-2\% increase in performance is the difference between life and death \cite{inbook}.

% These tradeoffs need to be considered during the model selection process. However, during model selection the data collection process is inefficient, i.e. collecting metrics on deep learning models requires compute resources.   

%Evaluation is a resource-intensive and time-consuming process as each model needs to be evaluated on each data point in the target dataset to determine how it will perform in operation.

\begin{figure}[tbp]
    \centering
    \includegraphics[height=2cm, width= \linewidth]{figures/selection_comparision.png}
    \caption{Model selection approaches: a) benchmark results (sub-optimal model selection), b) brute-force (wasteful API calls) and c) our proposed approach (balanced for target use case). Star indicates the optimal model for the target use case.}
    
    % Comparative analysis of model selection process, with the ideal model indicated by the star. Ad-hoc approach (left) evaluates models using their performance on a benchmark (but this is not always representative of performance on the target data). Brute force approach (middle) evaluates using all data on all models (but this is wasteful). Our approach (right) efficiently identifies a model suitable for the target usecase.
    
    
    \label{fig:selection_methods}
\end{figure}

% moved to introduction section as a hack to get the tool figure to show at the top of page 2.
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/Green-Runner-Overview.png}
    \caption{Overview of GreenRunnerGPT describing the internal processes and outputs from each process.}
    \label{fig:overview}
\end{figure*}

Model selection is currently an ad-hoc or wasteful process (see \autoref{fig:selection_methods}). Generally, the selection of ML models for building software applications can be broken down into three approaches, which are: i)The benchmark approach involves selecting models that perform well on a benchmark dataset and evaluating the best one on a target dataset. This approach finds sub-optimal models as benchmark datasets are not representative of every target dataset \cite{barbu2019objectnet}. 
In contrast, ii) the brute-force approach will result in a more accurate model but requires an extended evaluation of all models, which wastes resources (i.e. will result in an excessive number of model API calls, each of which consumes energy, to evaluate each model against each item in the target dataset) which increases development costs and iii) proxy metrics.

We refer to this problem as the evaluation tax -- paid by either sacrificing model performance or wasting energy consumed evaluating models that are not part of the final application resulting in incremental costs proportional to the number of candidate models. The problem of evaluation tax is a growing concern due to the increasing number of available deep-learning models. Hugging-face\footnote{https://huggingface.co/}, a popular model repository, has 198,613 models across 36 deep learning tasks all requiring evaluation and consideration of tradeoffs before use in the final application.

Prior work has proposed proxy metrics and selection strategies to reduce unnecessary computations during model selection, in particular, efficiently selecting models for the purpose of transfer learning or fine-tuning on a target dataset \cite{Renggli2022, Li2021}. However, these approaches focus solely on identifying the highest-performing model(s) rather than considering quality tradeoffs during the model selection process.

%\cite{Renggli2022}
%\cite{kornblith2019better,Pandy2022,zamir2018taskonomy,ge2017borrowing}
%\cite{deshpande2021linearized,you2021logme}

%To bridge this gap, we created GreenRunnerGPT to create an optimised model selection process (see \autoref{fig:selection_ours}).

To bridge this gap, we propose a novel tool, GreenRunnerGPT, for efficiently ML models \textit{balancing tradeoffs for a target use case}.
%The core idea is to help developers select a suitable model for their dataset in an energy-efficient manner, taking into account the tradeoffs involved and the metrics that need to be optimized for the target use case.
To support this process, we use a large language model (LLM) to suggest weights to assign to each quality indicator (accuracy, model complexity, model size, etc.) given a plain-text description of the target use case. These weights are used in the calculation of the reward function for a resource-efficient experimentation engine built upon a multi-armed bandit framework. Our approach efficiently evaluates models against the target dataset to determine the most promising models for the target use case with minimal evaluation tax. 



%Large language models have code generation abilities and are trained on internet scale datasets with technical blogs, code repositories, and technical papers. Our hypothesis is that within a large language model is sufficient knowledge of quality tradeoffs for deep learning applications that can be used to generate suitable configuration. This reduces the effort to create evaluation configuration, and to quantify competing trade-offs. GreenRunnerGPT is implemented to support model selection with an architecture that supports fine-tuning, hyperparameter optimisation, and machine learning API web services. 

In this paper, we demonstrate how  GreenRunnerGPT helps to 1) select the right quality indicators for a particular scenario and 2) reduce the carbon footprint of selecting a model that excels in those indicators.
% defined in \autoref{eq:reward}.
% \begin{equation}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}c@{}}
% $\text{reward} = \text{accuracy} \times \text{weight\_acc}$ \\[0.5em]
% $- \left(\dfrac{\log(\text{size}) - \log(\text{min\_size})}{\log(\text{max\_size}) - \log(\text{min\_size})}\right) \times \text{weight\_size}$ \\[0.5em]
% $- \left(\dfrac{\log(\text{complexity}) - \log(\text{min\_complexity})}{\log(\text{max\_complexity}) - \log(\text{min\_complexity})}\right) \times \text{weight\_complexity}$
% \end{tabular}%
% }
% \label{eq:reward}
% \end{equation}
% \begin{equation}
% \resizebox{\linewidth}{!}{%
% $\begin{aligned}
% \text{reward} &= \text{accuracy} \times \text{weight\_acc} \\
% &- \left(\dfrac{\log(\text{size}) - \log(\text{min\_size})}{\log(\text{max\_size}) - \log(\text{min\_size})}\right) \times \text{weight\_size} \\
% &- \left(\dfrac{\log(\text{complexity}) - \log(\text{min\_complexity})}{\log(\text{max\_complexity}) - \log(\text{min\_complexity})}\right) \times \text{weight\_complexity}
% \end{aligned}$%
% }
% \end{equation}

% With the tradeoffs suggested by the LLM, the selection process varies based on the user-determined use case by taking into account the metric weights for that use case as part of the reward function used to optimise the selection of model(s). \toolname currently integrates three MAB selection strategies: i) Epsilon Greedy, ii) Upper Confidence Bound, and iii) Thompson Sampling. These algorithms effectively balance exploration (by evaluating new models) and exploitation (by selecting the model with the highest reward) according to the specific requirements of the use case.
